Learning to Censor by Noisy Sampling

Point clouds are an increasingly ubiquitous input modality and the raw signal can be efficiently processed with recent progress in deep learning. This signal may, often inadvertently, capture sensitive information that can leak semantic and geometric properties of the scene which the data owner does not want to share. The goal of this work is to protect sensitive information when learning from point clouds; by censoring the sensitive information before the point cloud is released for downstream tasks. Specifically, we focus on preserving utility for perception tasks while mitigating attribute leakage attacks. The key motivating insight is to leverage the localized saliency of perception tasks on point clouds to provide good privacy-utility trade-offs. We realize this through a mechanism called Censoring by Noisy Sampling (CBNS), which is composed of two modules: i) Invariant Sampler: a differentiable point-cloud sampler which learns to remove points invariant to utility and ii) Noisy Distorter: which learns to distort sampled points to decouple the sensitive information from utility, and mitigate privacy leakage. We validate the effectiveness of CBNS through extensive comparisons with state-of-the-art baselines and sensitivity analyses of key design choices. Results show that CBNS achieves superior privacy-utility trade-offs on multiple datasets.

==> CBS/contrastive.tex <==
\section{Contrastive Loss}

% The reverse contrastive loss is given as:
% \begin{equation}
% \label{eq:contrasiveloss}
% \mathcal{L} = \frac{1}{2} \left( (1-y) \cdot (d_W)^2 + y \cdot (\max(0, m - d_W))^2 \right) \, ,
% \end{equation}
% Where $d_W$ is the Euclidean distance on the embedding space between the sample pair with $y = 1$ for a positive pair and  $y = 0$ when corresponding to a negative pair, and $m$ is the margin, empirically chosen to be \texttt{XXX}.

% For example, assume age is the sensitive variable. Unlike contrastive loss, where we encourage to pull positive samples (same age) closer within the local neighborhood and negative samples (different age) apart. In reverse contrastive loss, we map all different ages within a very small neighborhood of each other, in this way the adversary will experience confusion to select the correct age between different ages, leading to better privacy. In other words, the reverse contrastive loss forces to map the different ages to a single point in the feature space.

==> CBS/discussion.tex <==
\section{Dicussion}
We analyse the impact of key design choices for censoring by noisy sampling. Specifically, we study characterization of the sampler, noise transformer, objective function as well as the downstream perception network. For completeness, we also analyse the viability of line clouds for perception queries. For ease of exposition, we restrict scope of the analysis to the FaceScape dataset.

\subsubsection{Impact of Learned Sampling} We observe that task-dependent sampling significantly improves privacy-utility. This is evident from higher normalized hypervolume as well as better peak privacy-utility trade-offs. Specifically, (\textcolor{red}{compare numbers}) the peak-trade-off increases from $0.4333$ to $0.5043$ when a deterministic sampler is replaced with a learnt sampler (FaceScape). Results are presented in Table ~\ref{tab:ablate-sampler} \textcolor{red}{discuss both configs: whether to learn and how to learn.}

\begin{table}[]
\centering
\begin{tabular}{c|c|c|c}
\toprule
Technique   & Privacy ($\downarrow$) & Utility ($\uparrow$) & NHV ($\uparrow$) \\
\midrule
FS-LN                    & 0.9297   & 0.3954  & 0.1322 \\
LS-FN (ML)               & 0.6942  & 0.3602  & 0.1439 \\ % sn-gaussian
\midrule
CBNS (MaxEntropy)        & 0.6839  & 0.413   & 0.1596 \\ % sn-maxentropy
CBNS (ML)                & 0.5787  & 0.3638  & 0.1615 \\ % sn-adv
CBNS (ML + Rev-Contrast) & \textbf{0.5707}  & \textbf{0.3997}  & \textbf{0.1885} \\ % csn-pointwise discrim
\bottomrule
\end{tabular}
\caption{Sampling mechanism matters. Trade-off depends upon both of: i) whether transformation is learned, and ii) how it is learned. }
\end{table}

\subsubsection{Impact of Learned Noise} First, we observe that task-dependent noise significantly improves privacy-utility trade-offs. This is evident from higher normalized hypervolume as well as peak privacy-utility trade-off. Specifically, \textcolor{red}{compare numbers} the normalized hypervolume increases from $0.2730$ to $0.3258$ (FaceScape) upon learning the noise. Further, we also observe an increase in the peak tradeoff from $0.4175$ to $0.4791$ (FaceScape).  Next, we also observe that learning independent noise distribution for each sampled point is better as evident from improved fidelity. Previously, only affine transformation vs rotation of point cloud. \textcolor{red}{remark on invariance of pt set + weather is it learned and if learned pointwise.}

\begin{table}[]
\centering
\begin{tabular}{c|c|c|c}
\toprule
Technique   & Privacy ($\downarrow$) & Utility ($\uparrow$) & NHV ($\uparrow$)    \\
\midrule
LS - NN (ML)              & 0.5787  & 0.3638  & 0.1615 \\ % sn-adv
LS - FN (ML)              & 0.6942  & 0.3602  & 0.1439 \\ % sn gaussian
\midrule
CBNS (Shared, ML)         & 0.9051  & 0.4532  & 0.1586 \\ % sn-learnt
CBNS (Shared, ML + RC)    & 0.8600  & 0.4217  & 0.1625 \\ % csn-learnt
\midrule
CBNS (Pointwise, ML)      & \textbf{0.5689}  & \textbf{0.4013}  & 0.1530 \\ % sn pointwise discrim
CBNS (Pointwise, ML + RC) & \underline{0.5707}  & \underline{0.3997}  & \textbf{0.1885} \\ % csn pointwise discrim
\bottomrule
\end{tabular}
\caption{Learned Noise better, and significantly so when it is learned point-wise.}
\end{table}



% \subsubsection{Impact of Loss Function} Reverse Contrastive Objective is better. This is novel for visual signal, which we introduce. Prior methods extensive rely on some form of adversarial training -- either with a mix-max or max-entropy formalism. Unlike images, this achieves poor stability or trade-off for point clouds. We hypothesise this is due to sparse structure of the input signal. Beyond this work, this insight can be relevant for parallel efforts in generative point clouds ~\cite{generative-point-clouds} or adversarial attacks ~\cite{adv-attacks-pc}.

\subsubsection{Impact of Perception Network} We use both DGCNN and PointNet, two strong point cloud perception networks. We observe similar trends on privacy-utility trade-offs across baselines. Magnitude of normalized hypervolume also improves in DGCNN, which is a bigger backbone. Specifically, \textcolor{red}{add nos..}. Encouraging that our proposed sampling pipeline can generalize to several state-of-the-art networks. 

\begin{table}[]
\centering
\begin{tabular}{c|c|c|c|c}
\toprule
Technique              & Backbone      & Privacy ($\downarrow$) & Utility ($\uparrow$) & NHV \\
\midrule
\multirow{2}{*}{LS-FN} & PointNet & 0.6942  & 0.3602  &  0.1439   \\
                       & DGCNN    & 0.7056  & 0.4718  &  0.2136  \\
\midrule
\multirow{2}{*}{CBNS}  & PointNet & 0.5707  & 0.3997  & 0.1885  \\
                       & DGCNN    & 0.4848  & 0.4100  &  0.2361   \\
\midrule
\multirow{2}{*}{Line Cloud}  & PointNet & 0.5000  & 0.05  & -    \\
                       & DGCNN    & 0.5000  & 0.05  &  -   \\
                   
\midrule
\end{tabular}
\caption{Observed characteristic differences in saliency and capacity of different perception networks. Using DGCNN further improves performance over PointNet and helps achieve near optimal trade-off with our proposed CBNS. But, our noisy sampling technique is invariant to the type of network used by attacker. Also compare with resampling line clouds for perception}
\end{table}

\subsubsection{Infeasibility of Line Clouds} Perception networks cannot work with off-the-shelf line clouds because: i) networks are designed to leverage permutation invariance of unordered point clouds, ii) line clouds lack semantic information. Two possible baselines may occur: i) Resample line-clouds, ii) attack line-clouds. We experimentally compare with both. Resampling provides poor utility (random chance) and attacking provides poor privacy (when the point-cloud is retrieved) since the attack/defence mechanisms does not preserve semantic information. In fact, ii) is same as trivial no-privacy baseline, unless an additional intervention such as noisy sampling is applied.

==> CBS/formulation.tex <==
%Problem Formulation {Setup, Attack Model, Threat Model, Entities: Owner, Predictor, Adversary}; 
\section{Methodology}

\subsection{Preliminaries}

\subsubsection{Setup.}
Consider a dataset $D \in \mathbf{R}^{m\times n\times d}$ of $m$ point clouds, with each point cloud $P \in \mathbf{R}^{n\times d}$ defined as an unordered set of $n$ points with $d$ features. Corresponding to each $P$, there is a label set $Y \in \mathbf{R}^{\mu}$, consisting of $\mu$ attributes about the input. These attributes describe semantic information about the input, and may be represented as numerical or categorical variables. For instance, $P$ can be a facial point cloud with $Y$ being a set of attributes representing the face such as \textit{age, gender, expression}. With progress in machine learning, it is possible to train DNN models that can learn to predict (categorical) attributes $Y$ from raw point clouds $p$ ~\cite{point-cloud-classification}. In many scenarios, this paired dataset ($P, Y$) is captured locally on device and then released to an (untrusted) server that may train arbitrary predictive models $f(\theta; \cdot)$; where $f(\theta; P_{i}) : P \times \theta \longrightarrow Y$. Increasingly, considerations for balancing privacy and utility require that a data owner may want to keep some attribute $\hat{y} \in Y$ private, such that it cannot be: i) use to infer sensitive attributes $\hat{y}$ or, ii) be perceived using a pre-trained perception model for $\hat{y}$, with reasonable confidence and iii) allow for learning good models for perceiving attribute $y_1 \in {Y}/\hat{y}$. Consideration for balancing this privacy-utility trade-off has motivated work in private data release ~\cite{private-data-release} where a transformation $P' = T(P)$, is released instead of $P$. The goal of this work is to learn a censoring function $T$ that provides a good trade-off for perception queries. \textcolor{red}{to review.}

\subsubsection{Threat Model.}
Under our threat model, the untrusted server could attempt to learn the sensitive information by querying the point cloud dataset or training a state-of-the-art DNN model to predict $\hat{y}$ from $p$. For the evaluation and algorithm design purposes, we build a proxy adversary that attempts to approximate the worst-case real world adversary. This proxy adversary gets access to the paired dataset ($p', y$) is parameterized with an adversarial network $f_{adv}(\theta_a; \cdot)$ to predict the sensitive attribute $\hat{y}$
\subsubsection{Attack Model.}
The adversary may utilize the censored point cloud $p'$ to perform a leakage attack to infer the sensitive attribute. We adapt the standard supervised decoder attack model ~\cite{singh2021disco} where the adversary leverages a small number of $(p', \hat{y})$ pairs to train a decoder network $\hat{f}(\hat{\theta})$ such that $\hat{y}=\hat{f(p')}$. The practical validity of this attack is in the scenarios where some finite number of pairs $(p', \hat{y})$ is obtained by the server, and is hence valid in our setup where clients consent to sharing data with the server. This attack scheme is inspired by~\cite{dosovitskiy2016inverting,DBLP:journals/corr/MahendranV14,DBLP:journals/corr/TatarchenkoDB15}. Another practical scenario for this attack is where arbitrary pairs $(p', \hat{y})$ from the same data distribution is publicly available ~\cite{singh2021disco}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline_draft.png}
    \caption{Task setup we focus on. Censoring by Noisy Sampling to protect sensitive information when learning from point clouds. Three key entities: Client, Predictor and Adversary. Client transforms the dataset before releasing to the cloud, so that models can only learn to infer approved task information; while protecting sensitive information from adversary.
    }
    \label{fig:censor-by-sample}
\end{figure}

\subsubsection{Entities}
The problem of mitigating information leakage in point clouds is centered around three key entities: a data client, a predictor and an adversary. The client censors the point cloud dataset, to protect sensitive information, and releases it to the predictor which may use it to train model to infer sensitive attributes. An adversary is a semi-honest untrusted party (can be same as the predictor) which intercepts the released dataset with the intention to leak sensitive information.

\textbf{\underline{1. Data Client}} owns the point cloud dataset with sensitive information. The main objective for this data owner is to censor the sensitive information before the dataset is released to untrusted entities (predictor or adversary). The goal of any censoring mechanism is to ensure that the sensitive information is protected and cannot be learned from the released signal while also preserving utility of the signal for the predictor. Give an original dataset $p$, the client achieves this by releasing $r$ obtained from a transformation function ($T$) s.t. $r = T(p)$. Often, in practice, we observe that the design of $T$ depends upon the type of input signal and the intended set of queries it will be used for. The key contribution of this paper is a noisy sampler that helps achieve good privacy-utility trade-offs, when releasing point clouds for perception queries.

\textbf{\underline{2. Predictor}} is an untrusted entity which receives the released dataset ($r$) and queries it to extract information. We focus on perception queries -- we are non-linear queries focused on learning semantic attributes from the point cloud. We consider scenarios where the predictor trains a neural network to estimate such utility attribute(s). For classification tasks, predictor task network is optimized on a cross entropy objective function ($l_{cce}$). We note that transforming $p$ to release $r$ is challenging because the real predictor network is not accessible apriori, and can defined arbitrarily once the dataset is received. To learn the noisy sampler on-client, we mimic a proxy predictor assuming has access to $r$ and $y$. When dealing with sensitive attribute leakage, the task network assumes a state-of-the-art point cloud classification network.

\textbf{\underline{3. Adversary}} is a semi-honest entity that acquires access to the client dataset $r$ with the intent to leak the sensitive information. The challenge is to transform the dataset such that it can protect against attack by arbitrary adversary. To learn the noisy sampler on-client, we mimic a worst-case proxy adversary that obtains access to $r$ and $y$. When dealing with sensitive attribute leakage, the adversarial network assumes a state-of-the-art point cloud classification network.

\subsubsection{Privacy.}
Following the setup described by Hamm~\textit{et al.}~\cite{JMLR:v18:16-501}, we define privacy as the expected loss over the estimation of sensitive information by the adversary. This privacy loss $L_{priv}$, given $\ell_p$ norm, for an adversary can be stated as:
$$L_{priv}(\theta_1,\theta_3)\triangleq E[\ell_p(f_{adv}(f_s(p';\theta_1);\theta_3), \hat{y})]$$
Under this definition, releasing sensitive information while preserving privacy manifests as a min-max optimization between the data owner and the attacker. However, for training the model parameters, we use a proxy adversary from which gradients can be propagated. We refer the attack performed by this proxy adversary as \textit{online attack} and allows to mimic worst-case setups where the attacker can also dynamically adapt using protected data and sensitive label information ~\cite{singh2021disco}. We formalise our setup as an analogue but relax the non-invertibility assumption made by Hamm~\textit{et al.}~\cite{JMLR:v18:16-501} for the sampler  $f_{s}$, following \cite{DBLP:journals/corr/AroraLM15}, to generalize for potential attacks on sensitive inputs. We note that our definition of privacy significantly differs from differential privacy~\cite{dwork2006calibrating} since we aim to protect semantic attributes instead of identity of the data client.

==> CBS/method_backup.tex <==
\section{Methodology}
The proposed technique is visualized in figure ~\ref{fig:censor-by-sample} and detailed below. First, we introduce the attack and threat model and define the privacy considerations for our work. Next, we formalise the privacy evaluation setup and delineate our proposed method CBS, for protecting sensitive information in released point clouds.

\subsection{Formulation}
% Setup: Dataset at client. Inputs + labels. Released to third person to train arbitrary models. Goal --> how to remove sensitive information --> so sensitive attribute cannot be inferred. Need private data release.
\subsubsection{Setup.}
Consider a dataset $D \in \mathbf{R}^{m\times n\times d}$ of $m$ point clouds, with each point cloud $P \in \mathbf{R}^{n\times d}$ defined as an unordered set of $n$ points with $d$ features. Corresponding to each $P$, there is a label set $Y \in \mathbf{R}^{\mu}$, consisting of $\mu$ attributes about the input. This attributes can describe semantic information about the input, and may be represented as numerical or categorical variables. For instance, $P$ can be a facial point cloud with $Y$ being a set of attributes representing the face such as \textit{age, gender, expression}. With progress in machine learning, it is possible to train DNN models that can learn to predict (categorical) attributes $Y$ from raw point clouds $p$ ~\cite{point-cloud-classification}. In many scenarios, this paired dataset ($P, Y$) is captured locally on device and then released to an (untrusted) server that may train arbitrary predictive models $f(\theta; \cdot)$; where $f(\theta; P_{i}) : P \times \theta \longrightarrow Y$. Increasingly, considerations for balancing privacy and utility require that a data owner may want to keep some attribute $\hat{y} \in Y$ private, such that it cannot be: i) use to train perception models for $\hat{y}$ or, ii) be perceived using a pre-trained perception model for $\hat{y}$, with reasonable confidence and iii) allow for learning good models for perceiving attribute $y_1 \in {Y}/\hat{y}$. Consideration for balancing this privacy-utility trade-off has motivated work in private data release ~\cite{private-data-release} where a transformation $P' = T(P)$, is released instead of $P$. The goal of this work is to learn censoring function $T$ that have provide good trade-offs for perception queries. \textcolor{red}{to review.}

\subsubsection{Threat Model.}
Under our threat model, the untrusted server could attempt to learn the sensitive information by querying the point cloud dataset or training a state-of-the-art DNN model to predict $\hat{y}$ from $p$. For the evaluation and algorithm design purposes, we build a proxy adversary that attempts to approximate the worst-case real world adversary. This proxy adversary gets access to the paired dataset ($p', y$) is parameterized with an adversarial network $f_{adv}(\theta_a; \cdot)$ to predict the sensitive attribute $\hat{y}$
\subsubsection{Attack Model.}
The adversary may utilize the censored point cloud $p'$ to perform a leakage attack to infer the sensitive attribute. We adapt the standard supervised decoder attack model ~\cite{disco} where the adversary leverages a small number of $(p', \hat{y})$ pairs to train a decoder network $\hat{f}(\hat{\theta})$ such that $\hat{y}=\hat{f(p')}$. The practical validity of this attack is in the scenarios where some finite number of pairs $(p', \hat{y})$ is obtained by the server, and is hence valid in our setup where clients consent to sharing data with the server. This attack scheme is inspired from~\cite{dosovitskiy2016inverting,DBLP:journals/corr/MahendranV14,DBLP:journals/corr/DosovitskiyB15}. Another practical scenario for this attack is where arbitrary pairs $(p', \hat{y})$ from the same data distribution is publicly available ~\cite{disco}.
\subsubsection{Privacy.}
Following the setup described in Hamm~\textit{et al.}~\cite{JMLR:v18:16-501}, we define privacy as the expected loss over the estimation of sensitive information by the adversary. This privacy loss $L_{priv}$, given $\ell_p$ norm, for an adversary can be stated as:
$$L_{priv}(\theta_1,\theta_3)\triangleq E[\ell_p(f_{adv}(f_s(p';\theta_1);\theta_3), \hat{y})]$$
Under this definition, releasing sensitive information while preserving privacy manifests as a min-max optimization between the data owner and the attacker. However, for training the model parameters, we use a proxy adversary from which gradients can be propagated. We refer the attack performed by this proxy adversary as \textit{online attack} and allows to mimic worst-case setups where the attacker can also dynamically adapt ~\cite{disco}. We formalise our setup as an analogue but relax the non-invertibility assumption made by Hamm~\textit{et al.}~\cite{JMLR:v18:16-501} for the sampler  $f_{s}$, following \cite{DBLP:journals/corr/AroraLM15}, to generalize for potential attacks on sensitive inputs.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{example-image-b}
    \caption{Censoring by Noisy Sampling to protect sensitive information when learning from point clouds.}
    \label{fig:censor-by-sample}
\end{figure}

\subsection{Censoring by Sampling}
\textit{CBS}, depicted in figure ~\ref{fig:censor-by-sample} is composed of three key entities: a client, a predictor and an adversary. The client transforms the point cloud dataset, to censor sensitive information, and releases it to the predictor which may use it to train model to infer sensitive attributes. An adversary is a semi-honest untrusted party (can be same as the predictor) which intercepts the released dataset with the intention to leak sensitive information.

\subsubsection{Data Client} owns the point cloud dataset with sensitive information. The main objective for this data owner is to censor the sensitive information before the dataset is released to the server. We introduce a noisy sampling mechanism for this censoring. Given an input point cloud $p$, the released point cloud $r$ is obtained as $r = f_n(f_s(p))$. Here $f_n(\theta_n; \cdot)$ and $f_s(\theta_s; \cdot)$ are parameterized functions.

\subsubsection{Predictor} is an untrusted entity which receives the released point cloud $r$ and trains a task network to estimate the task attribute(s). For classification task, the task network is optimized on a cross entropy objective function ($l_{cce}$). To learn the noisy sampler on-client, we mimic a proxy predictor that has access to $r$ and $y$. The task network assumes a state-of-the-art point cloud classification network optimized using $l_{cce}$.

\subsubsection{Adversary} \label{sec:adversary} is a semi-honest entity that acquires access to the client dataset $r$ and trains an adversarial network with the intent to leak the sensitive information. To learn the noisy sampler on-client, we mimic a proxy adversary that obtains access to $r$ and $y$. The adversarial network assumes a state-of-the-art point cloud classification network optimized using $l_{cce}$

\subsection{Training}
The sampler can be trained by: i) data-owning client, ii) trusted intermediary server (when total dataset is distributed across clients).
In this scenario, the noisy sampler is trained. Let the proxy adversary encoder ($a$) be a parameterized function $a(\theta_{a}; .)$ that produces a compressed representation of the input. And let $y_{t}, y_{s}$ be task-specific labels and sensitive labels respectively. Then the loss function can be defined as:

% key idea is to increase the distance between features of same sensitive class and decrease the distance between the features of different sensitive class: ie opposite of contrastive learning for sensitive attributes


\begin{align}
    L =(\lambda_{1} * L_{sampler}) + (\lambda_{2} * L_{adv}) - (\lambda_{3} * L_{cont}) \\
    L_{adv} = \alpha * (l_{cce}(r, y_{t})) + (1 - \alpha) * (l_{cce}(r, y_{s})) \\
    L_{cont} = D(a(r), a(r_{pos}))^{2} - D(a(r), a(r_{neg}))^{2}
\end{align}

Where $r, r_{pos}, r_{neg}$ are the anchor, positive and negative for the contrastive loss ($L_{cont}$) and $D$ represents euclidean distance between the attack-specific $a$ features of the inputs. Note that $r_{pos}, r_{neg}$ are randomly sampled from the training dataset and are examples of same sensitive class and different sensitive class as $r$ respectively. Sampler loss ($L_{sampler}$) is same as in \cite{lang2020samplenet}. The gradients of the proposed loss jointly optimize a) Task network b) $f_s$ c) $f_n$ (\textcolor{red}{rephrase})



==> CBS/prelim.tex <==
\section{Background}
This section draw from background work to motivate our setup, constraints and the proposed technique.

\subsection{Saliency of Point Clouds}
Empirical analysis of point cloud networks shows that perception of a specific attribute only depends upon a small subset of the total points. This localized saliency is a key motivating insight for our work. In principle, we can have good privacy and utility by only keep points corresponding to the utility attribute. Interestingly, the set is non-unique because a combination of invariant and overlapping set. However, in practice we note that there exists a privacy-utility \textit{trade-off} since the localization of sensitive and task attributes can overlap. Thus, we introduce mechanisms for task-dependent noisy sampling to achieve good and tunable trade-offs. \textcolor{red}{cartoon for invariant + overlapping sets; viz localized receptive fields for perception; stats}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{example-image-b}
    \caption{\textbf{Premise Validation}: Localized Saliency of Point Clouds w Non-Overlapping sets. Cartoon + viz + statistics}
    \label{fig:saliency-fig}
\end{figure}

\subsection{Noisy Sampling for Conditional Privacy}
Noisy sampling has previously been explored at the intersection of computational geometry and privacy - specifically private coresets. This work on focusing on publishing sanitizer versions of datasets -- which presere differential privacy can be queried ad infinitum without impacting privacy. Various mechanisms have been introduced - without loss of generality - propose some combination of two steps: i) selecting a viable subset (coreset), ii) adding differentially-private noise to the coreset (privacy). However, methods have only focused on tabular datasets with linear queries (eg. mean, median), where existing tools in the DP-framework to compute noise sensitivity of the queries and provide guarantees. However, in contrast, we work with visual (point cloud) datasets where queries involve training neural networks (over multiple iterations) and hence are highly non-linear and non-ergodic (iterative). Estimating DP-noise sensitivity of neural network is an open problem. We note that training with DP-SGD is not amenable as it adds noise to the gradients (or model weights) and protects the trained model, not the dataset as required here.
However, our mechanism follows a similar pipeline for noisy sampling and we validate good privacy-utility trade-offs through extensive empirical analysis.

==> CBS/premise.tex <==
\section{Premise Validation}
% Key Insight - subset of critical points that guide decision. this localized saliency is task-oriented. Non-unique and a network can be trained to learn to identify them. Example and Intuition: Venn-diagram
%for privacy-utility: need to remove points that: a) not important for utility [invariant sampler], b) relevant for privacy [noisy deformer]. Motivates need for mechanisms for noisy sampling. Which we will introduce in the next section.
% Remark of Noisy Sampling for Conditional Privacy: Similar work not for visual point clouds but for tabular datasets. Private Coresets: some combination of subset selection and differentially-private noise. But, only support linear queries. We are different: i) non-linear queries: need DNN models + can't compute sensitivity, ii) visual signal.

The main contribution of this paper is designing transformation functions that can censor  sensitive information before the dataset is released to untrusted servers. Specifically, we propose to achieve this - for point clouds - through a noisy sampler, to achieve good trade-off on privacy (censoring) and utility. In this section, we motivate the validity of our hypothesis and discussing specific constraints. The intended takeaways are: i) why to sample and with noise? ii) the specific technique we use.

\subsubsection{Saliency of Point Clouds.}
Empirical analysis of point cloud networks shows that perception of a specific attribute only depends upon a small subset of the total points. This localized saliency is a key motivating insight for our work. In principle, we can have good privacy and utility by only keep points corresponding to the utility attribute. Interestingly, the set is non-unique because a combination of invariant and overlapping set. However, in practice we note that there exists a privacy-utility \textit{trade-off} since the localization of sensitive and task attributes can overlap. Thus, we introduce mechanisms for task-dependent noisy sampling to achieve good and tunable trade-offs. \textcolor{red}{cartoon for invariant + overlapping sets; viz localized receptive fields for perception; stats}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Premise_Validation_fig.png}
    \caption{\textbf{Premise Validation}: a) There exist critical points that guide perception, and are specific to task b) Point subset can overlap for different tasks. c) Quantitative metrics of overlap between two different tasks on the same point cloud. Noisy sampling of the point set can help trade-off privacy and utility. \textcolor{red}{Cartoon + viz + statistics}}
    \label{fig:saliency-fig}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/sampling_examples.pdf}
    \caption{\textcolor{red}{Need to change representation.}}
    \label{fig:sampling-examples}
\end{figure}

\subsubsection{Noisy Sampling for Conditional Privacy.}
Noisy sampling has previously been explored at the intersection of computational geometry and privacy, through research in private coresets ~\cite{private-coresets}. This field of work focuses on publishing sanitized versions of datasets -- which preserve differential privacy can be queried ad infinitum without impacting privacy. Various mechanisms have been introduced - without loss of generality - propose some combination of two steps: i) selecting a viable subset of input features (coreset), ii) adding differentially-private noise to the coreset (privacy). However, methods have only focused on tabular datasets with linear queries (eg. mean, median), where existing tools in the DP-framework to compute noise sensitivity of the queries and provide guarantees. However, in contrast, we work with visual (point cloud) datasets where queries involve training neural networks (over multiple iterations) and hence are highly non-linear and non-ergodic (iterative). The key differences of our work, from prior work in private coresets is: a) subset of visual signal to select rows, ii) non-linear queries with neural networks. Estimating DP-noise sensitivity of neural network is an open problem. We note that training with DP-SGD is not amenable as it adds noise to the gradients (or model weights) and protects the trained model, not the dataset as required here. However, our mechanism follows a similar pipeline for noisy sampling and we validate good privacy-utility trade-offs through extensive empirical analysis. \textcolor{red}{to review.. make clear}

==> CBS/results_backup.tex <==
\section{Results and Discussion}

\subsection{Comparison with Baselines}
Performance is reported in Tables ~\ref{tab:facescape-main} and ~\ref{tab:modelnet4-main} along the two key dimensions: peak privacy-utility trade-offs and normalized hypervolume. Results in Table ~\ref{tab:facescape-main} show that CBS significantly outperforms all baselines, as evident from the higher normalized hypervolume. This is also corroborated by a superior peak privacy-utility trade-off which is achieved. Specifically, we observe that \textcolor{red}{all specific values + compare with the default no-privacy setup} 

% We report peak privacy-utility trade-off and the normalized hypervolume. Higher value is better. Trade-off various techniques for noisy sampling. Key insight: both sampling and noise transformer are key. From Table ~\ref{tab:modelnet4-main} more sensitive to noise transformer than sampling strategy. But, learned noise is better than task noise. We visualize the privacy-utility trade-off in figure ~\ref{fig:facescape-mainfig}. 


\begin{table}
\centering
\begin{tabular}{cccccc} 
\toprule
\begin{tabular}[c]{@{}c@{}}\\\textbf{Method}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{No. of}\\\textbf{Points}\end{tabular} & \multicolumn{4}{c}{\textbf{Accuracy}} \\ 
\midrule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Expression} & \textbf{Gender} & \textbf{Identity} & \textbf{Age} \\ 
\midrule
PointNet & 1024 & 0.5877 & 0.9693 & 0.9870 & 0.9852 \\
DGCNN & 1024 & 0.6409 & 0.9493 & - & - \\
FPS & 64 & 0.4003 & 0.9375 & 0.9432 & 0.9393 \\
\begin{tabular}[c]{@{}c@{}}Learnt Sampler\\(PointNet)\end{tabular} & 64 & 0.4549 & 0.9515 & 0.9625 & 0.9691 \\
\begin{tabular}[c]{@{}c@{}}Learnt Sampler\\(DGCNN)\end{tabular} & 64 & 0.4797 & 0.9349 & - & - \\
\bottomrule
\end{tabular}
\caption{Classification performance on FaceScape dataset.}
\end{table}

\begin{table}
\centering
\begin{tabular}{cccc} 
\toprule
\begin{tabular}[c]{@{}c@{}}\\\textbf{Method}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{No. of}\\\textbf{Points Sampled}\end{tabular} & \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
\midrule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \begin{tabular}[c]{@{}c@{}}\textbf{Living/}\\\textbf{Non-Living}\end{tabular} & \textbf{Modelnet Class} \\ 
\midrule
PointNet & 2048 & 0.98125 & 0.9375 \\
\multicolumn{1}{l}{FPS (PointNet)} & 64 & 0.93812 & 0.90625 \\
\begin{tabular}[c]{@{}c@{}}Learnt Sampler\\(PointNet)\end{tabular} & 64 & 0.962500 & 0.95 \\
\bottomrule
\end{tabular}\
\caption{Classification performance on ModelNet dataset.}
\end{table}

\begin{table}
\centering
\begin{tabular}{ccccc} 
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{ Method }\end{tabular} & \textbf{1 - HV} & \begin{tabular}[c]{@{}c@{}}\textbf{Privacy}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Task Acc}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Best Tradeoff}}\\\textbf{\textbf{(Task / Sensitive)}}\end{tabular} \\ 
\hline
FPS Gaussian & 0.2072 & 0.04884 & 0.4122 & 0.43337 \\
FPS Learnt & 0.2199 & 0.05233 & 0.40955 & 0.43217 \\
FPS Pointwise & 0.1276 & 0.06023 & 0.38750 & 0.41234 \\ 
\hline
SN Gaussian & 0.2642 & 0.28573 & 0.36021 & 0.50431 \\
SN Max Entropy & 0.3016 & 0.29607 & 0.41311 & 0.58687 \\
SN & 0.2961 & 0.40125 & 0.36381 & 0.60762 \\
SN Learnt & 0.3328 & 0.15523 & 0.42266 & 0.50033 \\
SN Pointwise & 0.2294 & 0.41103 & 0.40135 & \textbf{0.68145} \\ 
\hline
Contrastive &  & 0.12884 & 0.44970 & 0.51621 \\
CSN Gaussian & 0.2730 & 0.47942 & 0.21734 & 0.41750 \\
CSN Learnt & 0.3258 & 0.11990 & 0.42171 & 0.47916 \\
\textbf{CSN Pointwise} & \textbf{0.3919} & 0.40920 & 0.39974 & \textbf{0.67662} \\
\bottomrule
\end{tabular}
\caption{PointNet FaceScape}

\end{table}

\begin{table}
\centering
\begin{tabular}{ccccc} 
\toprule
\begin{tabular}[c]{@{}c@{}}\\\\\\\textbf{ Method }\end{tabular} & \textbf{1 - HV} & \begin{tabular}[c]{@{}c@{}}\textbf{Privacy}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Task Acc}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Best Tradeoff}}\\\textbf{\textbf{(Task / Sensitive)}}\end{tabular} \\ 
\hline
SN Max Entropy & 0.81365 & 0.10312 & 0.875 & 0.97560 \\
SN & 0.827987 & 0.078125 & 0.875 & 0.9491525 \\
SN Gaussian & 0.77226 & 0.6875 & 0.61875 & 1.98 \\
SN Learnt & 0.74919 & 0.80937 & 0.55312 & \textbf{2.901639 } \\
SN Pointwise & 0.76797 & 0.6656 & 0.62812 & 1.878504 \\ 
\hline
Contrastive & 0.51623 & 0.0999 & 0.84062 & 0.934027 \\
CSN Gaussian & 0.77366 & 0.7218 & 0.625 & 2.247191 \\
CSN Learnt & 0.69026 & 0.73437 & 0.675 & \textbf{2.541176 } \\
CSN\textbf{ }Pointwise & 0.707723 & 0.69375 & 0.628125 & 2.051020 \\
\bottomrule
\end{tabular}
\caption{PointNet ModelNet}
\end{table}


\begin{table}
\centering
\begin{tabular}{ccccc} 
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{ Method }\end{tabular} & \textbf{1 - HV} & \begin{tabular}[c]{@{}c@{}}\textbf{Privacy}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Task Acc}\\\textbf{(Best Tradeoff)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Best Tradeoff}}\\\textbf{\textbf{(Task / Sensitive)}}\end{tabular} \\ 
\hline
SN Gaussian & 0.31162 & 0.29478 & 0.47180 & 0.6690 \\
SN Learnt & 0.25499 & 0.15105 & 0.46220 & 0.54442 \\
SN Pointwise & 0.35796 & 0.43751 & 0.44701 & 0.79118 \\ 
\hline
\textbf{CSN Pointwise} & \textbf{0.48126} & 0.49517 & 0.41000 & \textbf{0.81228} \\
\bottomrule
\end{tabular}
\caption{DGCNN Facescape}
\end{table}

